From Priest to Doctor: Domain Adaptation for Low-Resource Neural Machine Translation

Many of the world's languages have insufficient data to train high-performing general neural machine translation (NMT) models, let alone domain-specific models, and often the only available parallel data are small amounts of religious texts. Hence, domain adaptation (DA) is a crucial issue faced by contemporary NMT and has, so far, been underexplored for low-resource languages. In this paper, we evaluate a set of methods from both low-resource NMT and DA in a realistic setting, in which we aim to translate between a high-resource and a low-resource language with access to only: a) parallel Bible data, b) a bilingual dictionary, and c) a monolingual target-domain corpus in the high-resource language. Our results show that the effectiveness of the tested methods varies, with the simplest one, DALI, being most effective. We follow up with a small human evaluation of DALI, which shows that there is still a need for more careful investigation of how to accomplish DA for low-resource NMT.

==> sections/old_paper.tex <==
\begin{abstract}
Domain adaptation (DA) is a challenging but crucial issue faced by contemporary approaches to Neural Machine Translation (NMT), and even more so for low-resource languages.
For many of the world's languages, there is insufficient parallel data to train high-performing general NMT models, let alone domain-specific models, and often the only available parallel data are from a very narrow religious domain.
In this paper, we \st{apply} \amcomment{evaluate} existing methods from both low-resource NMT and DA to a realistic low-resource setting, in which we have access to \amcomment{only}: a) restricted parallel data, b) a bilingual dictionary, and c) a monolingual target-domain corpus for the high-resource source language.
\amcomment{Our results  - which represent the first application of these methods to this setting - \st{show that the approaches fail to produce usable target-domain NMT systems, calling for more careful investigation of how to accomplish domain adaptation in the low-resource NMT setting.  } demonstrate the varying benefits of the methods under study, where the simplest proves most effective. Additionally, we aim to emphasize the need for a more careful investigation of how to accomplish domain adaptation in the low-resource NMT setting.}

% Our results - the first for application of these methods to this setting - show that the approaches fail to produce usable target-domain NMT systems, calling for more careful investigation of how to accomplish domain adaptation in the low-resource NMT setting.
\end{abstract}

\section{Introduction}

Neural machine translation models have shown remarkable performance when trained on large datasets,
%However, they demonstrate 
but they have limited ability to deal with low-resource languages that lack large scale monolingual and parallel corpora %for model training
\cite{wang2021survey}. Moreover, NMT systems face challenges when translating text from a novel domain characterized by a unique style or vocabulary \cite{koehn-knowles-2017-six, saunders2022domain}. Often, these issues co-occur, a scenario that has so far has been neglected by researchers. 
Most of the world's 7000+ languages are considered low-resource \cite{joshi2020state}, and the existing data for them are in limited domains; languages that could most benefit from domain adaptation are the ones left behind. 

In this paper we explore the realistic setting where we are restricted to 
%utilize 
only commonly available resources: a limited parallel corpus in the source domain (e.g. religious texts), monolingual target-domain texts in the high-resource language, 
%that is also in the domain of interest (target domain), 
and a bilingual dictionary for the two languages.
\amcomment{Many languages do not even have a related high-resource language to utilize here,\footnote{Like many languages of North and South America.\amcomment{TODO: need citation}} thus making the limited resources we have chosen a generalizable setting to many truly low-resource languages. As finding data in different domains for truly low-resource languages proved difficult, we \textit{simulate} these settings by using a base multilingual model that was not pre-trained on them. }
%that ideally covers the in-domain terms of the target domain. 

%\ermargincomment{With these limitations in place, we experiment with methods in translating from English to a simulated low-resource target language.}
% We probe this setting by inspecting some methods for domain adaptation when translating from English to some low-resource language.
With these constraints in place, we experiment with 
%different 
\amcomment{some of the }existing domain adaption and low-resource NMT methods, translating from English to a simulated low-resource target language. 
We use pre-trained mBART \cite{liu-etal-2020-multilingual-denoising}
as our base model, fine-tune on parallel Bible texts, and target the domains of government and medical documents.
%Our (source-domain) parallel corpora are exclusively biblical verses, and our 
%For the 
%target domains 
%we examine both 
%are government and medical documents.
%, while the only parallel corpora we have access to are biblical verses. 
%We use mBART \cite{liu-etal-2020-multilingual-denoising} as the base model \lgmargincomment{combine with the sentence two before this to avoid redundancy} and implement some different methods on top of it. 
The methods we investigate use the bilingual dictionaries in various ways.
%All these methods use a bilingual dictionary, but all in different aspects. The target languages are not low-resource; however, they are not used in mBART's pre-training and can hence to some extent simulate an actual low-resource language. 
%\apmargincomment{Add description of experimental set-up/method/approach} \ammargincomment{Is this something?}

Our results showcase the \amcomment{\st{limited} varying} effectiveness of existing methods for the realistic setting of building a domain-specific NMT system for a low-resource language without parallel domain-specific data. \amcomment{The simplest approach which roughly does word-replacement with forward-translation yields the best gains on average.}

%proposed setting. To the best of our knowledge, no existing work directly studies domain adaptation in NMT for low-resource languages in this setting. Thus, the methods either were proposed for "domain adaptation in NMT" or "low-resource NMT". 


\section{Related Work}
In this study we investigate methods from both low-resource NMT and DA for NMT.

\paragraph{Domain Adaptation in NMT.}
Because domains are defined by the characteristics of data \cite{saunders2022domain}, some of the most effective approaches focus on the data, and thus 
%alone rather than the underlying  architecture \apmargincomment{be more specific}\ammargincomment{hope this is clearer}, as domains are defined by the characteristics of data \cite{saunders2022domain}. 
can be applied to various underlying architectures.
% One approach involves extending training data by retrieving general-domain examples that resemble the target-domain
% \cite{xu-etal-2020-boosting, poncelas-etal-2019-transductive, cai-etal-2021-neural, vu2021machine}. 
% A group of approaches 
Some works focus on acquiring monolingual in-domain data, which is generally easier
%is usually much more convenient 
than finding in-domain parallel data. Back-translation uses authentic monolingual target-domain data in the
%in the target domain and 
target language and produces artificial source sentences using 
%relies on 
a target-to-source neural NMT model \cite{poncelas2019adaptation, jin2020simple}.
%When data in the target language and target domain is available, synthetic source-side data can be produced  There are some approaches that make 
Another approach uses monolingual source-side corpora and a source-to-target NMT model for forward-translation, 
where it is common to employ self-learning \cite{chinea-rios-etal-2017-adapting}. 
% \cite{gordon-duh-2020-distill} use one or several stronger teacher models, training or tuning a smaller student model on their outputs. 
With access to a small parallel corpus, extra training data can be created by introducing noise, which improves the robustness of MT models \cite{vaibhav-etal-2019-improving}. Synthetic parallel data can be acquired from an external source or generated using a predefined or induced lexicon. \citet{dali} use a lexicon to back-translate target-side sentences. \citet{peng2020dictionary} use a dictionary for data augmentation, injecting dictionary terms at appropriate parts of out-of-domain texts to synthesize in-domain training data. \amcomment{\citet{bergmanis-pinnis-2021-facilitating} augment the training data by annotating randomly selected source language words with their target language lemmas to integrate terms.}
\citet{zhang-etal-2022-iterative} introduce lexical constraints into iterative back-translation. 


Other approaches add parameters to the model, for example adding domain tags, introducing extra tag embeddings, or even submodules
%Some of these label the domains - using tags - which could introduce extra embeddings for the tags, or even submodules
\cite{kobus-etal-2017-domain,stergiadis-etal-2021-multi}. This manipulation of the embeddings could extend to more terms in the vocabulary, beyond the tags \cite{pham-etal-2019-generic,sato-etal-2020-vocabulary, man2023wdsrl}.
% Auxiliary trainable subnetworks could be added to the model \cite{lin-etal-2021-towards}.
%It could be in the form of 
With adapter-based methods, a domain-specific module is trained, freezing other parameters for more efficient training \cite{bapna-firat-2019-simple}. \citet{leca} add a pointer-generator module to copy from suggestions in the input, where the suggestions are drawn from a domain-specific dictionary. 

\paragraph{Low-Resource NMT.}
 Approaches targeting low-resource MT show some overlap with domain adaptation methods, as a new language can be viewed as an extreme case of a new domain. One popular approach is data augmentation, which can be in the form of word or phrase replacement with the help of a bilingual lexicon \cite{nag2020incorporating}. Back-translation, forward-translation and data selection methods could still be applied \cite{sennrich-etal-2016-improving, fadaee-monz-2018-back, dou-etal-2020-dynamic}. Transfer Learning is a useful technique in low-resource NMT \cite{10.1145/3314945, kocmi-bojar-2020-efficiently, cooper-stickland-etal-2021-recipes}. 
\citet{liu-etal-2021-continual} continually pre-train mBART \cite{liu-etal-2020-multilingual-denoising} on unseen languages, slightly changing the pre-training objective to utilize a bilingual dictionary. 
% Some semi-supervised approaches include using monolingual data to create language models \cite{gulcehre2015using} and multi-task learning \cite{domhan-hieber-2017-using}. However, they require a large amount of monolingual texts which still be unfeasible for low-resource languages. 
Although we do not inspect large language models in our experiments for domain adaption, some recent works hint at the potential of LLMs for low-resource machine translation. \amcomment{\citet{robinson-etal-2023-chatgpt} observe that ChatGPT's machine translation capabilities across the 204 languages of the FLORES-200 dataset \cite{costa2022no} consistently lags behind traditional machine translation models in the case of low-resource languages.} \citet{ghazvininejad2023dictionary} use dictionaries to suggest words for the model to use in the output translation.
%give the model some suggestions for the words to use in the output translation, while giving the model some examples of the translation
\citet{zhang2024teaching} improve their model by adopting different strategies for dictionary term lookup and the retrieval of examples for in-context learning.
\citet{siddhant2022towards, 10.1145/3567592} note that, in the case of many low-resource languages, the problem is more severe since the only available parallel data are religious texts.


\section{Data}
For all experiments, the only source of parallel data we use \textit{as parallel data} is the JHU Bible Corpus
%In all the experiments, we limit ourselves to The John Hopkins University Bible Corpus 
\cite{mccarthy-etal-2020-johns}. 
%as our only source of parallel data. 
We \amcomment{separately} adapt to two different domains: government and medical texts.
Because of the difficulty of sourcing domain-specific data in truly low-resource languages, we simulate a low-resource setting, selecting languages not seen by mBART during pre-training.
%Note that while most of these languages are not truly low-resource, the pre-trained model has not seen them during pre-training and they can therefore serve as acceptable substitutes for low-resource languages. One of the main hurdles of finding a more appropriate low-resource language is the availability of data in different domains. 
For the government domain, we conduct experiments on Croatian, Icelandic, Maltese, Polish, and Ukrainian. For the medical domain, we 
%do the same set of experiments for 
use Croatian, Icelandic, Maltese, and Polish. The domain-specific data mostly come from past WMT translation tasks.
%for government and medical data. 

Given our experimental settings (Section~\ref{sec:exp}), training and pre-training stages use only source-side sentences from these parallel data sets.\footnote{We could of course use other monolingual data sources, but we use (mostly) WMT data for experimental flexibility.}
% \apmargincomment{The argument for not using external data wasn't really convincing - I made a different justification, but I'm not sure that this one is convincing either.}
Data availability varies across language/domain pairs, and we cap data set sizes to maintain comparability across languages.
For \textbf{training} we use no more than 200K sentence pairs.
If our setting requires \textbf{pre-training}, we use the same source-side sentences used for training.
\textbf{Test} data sets for all settings consist of 1500 sentence pairs.



%As will be discussed in Section \ref{sec:exp}, there are two stages we might need data for in different settings: training and pre-training, and in both cases we only need the source-side sentences. We use 1500 sentence pairs as the test split in all the settings, and no more than 200K sentence pairs for training (and if the setting does require pre-training, we use the same source-side sentences that we used for training for pre-training as well). %There are varying levels of availability of data for different domains in different languages, and that is why we do not use more than 200K sentences: for the different experiments to be roughly comparable. 
%Note that we can use some irrelevant source-side text in the target domain for both training and pre-training as well, but we hypothesized that using the source-side
%data from a corpus that translated already, might yield some more relevant data in regard to the target language and the people using that language; as the data was translated because it \textit{probably} needed to be translated. 
More details about the data used for each domain and language pair can be found in Appendix \ref{sec:app-data}.
%\lgmargincomment{this is a huge graf, try to break it up if you can}

\paragraph{Dictionaries.}
\label{dict:making}
The methods we investigate here call for bilingual (source-target language) dictionaries.
To build dictionaries, for each language pair we extract the 5000 most frequent lemmas, together with their inflections, from the training data and use the Google Translate API\footnote{\url{https://cloud.google.com/translate/}} to translate those words.
We expect that performance might increase if we had access to domain-specific bilingual dictionaries for each language pair.
%A bilingual dictionary is used for each of our approaches. We hypothesize that if the dictionary is in-domain we would see larger boosts in performance;
% This dictionary is preferably \lgmargincomment{you should clarify if this preference is just based on your intuitions or if the previous works you're reproducing say this} an in-domain one;%
%so if the target domain of translation is the medical domain, the dictionary would contain medical terms which would hopefully help the model with rare domain-specific vocabulary. 
%Instead of finding in-domain dictionaries for these target languages and domains, we extract the most frequent lemmas ($N=5000$) and their respective inflections on the source side of the training split, and use the Google Translate API\footnote{\href{https://cloud.google.com/translate/}{https://cloud.google.com/translate/}} to make up a dictionary.\lgmargincomment{If this is common practice for getting a dictionary like this it might be helpful for your presentation to say so}\ammargincomment{I don't think it is, but I did it cause it made sense. I don't know of any other paper that makes dictionaries with google translate.}

We augment this dictionary with word pairs extracted from our small parallel corpora, using standard statistical approaches for lexicon induction. 
Specifically, we employ Fast Align \cite{dyer-etal-2013-simple} on the Bible verses.% to complement the previous dictionary with new entries. 
The expansion of the dictionary with statistical methods follows previous work \cite{dali, zhang2024teaching}. Further information about the dictionaries is available in Appendix \ref{sec:app-dict}.


\section{Experimental Setup} 
\label{sec:exp}
% \apcomment{Add an overview of the experimental approach, explaining the overall shape of the experiments}
The core task is translation from a high-resource language (English in our case) into a low-resource language, investigating one baseline and four different modeling approaches, described below. All settings use mBART as the backbone model 
%for all experiments 
and are implemented 
%all methods 
using
\texttt{fairseq}.\footnote{\url{https://github.com/facebookresearch/fairseq}}

The different settings vary in how they use the available resources (parallel Bible data, monolingual source data, and bilingual lexicons), \amcomment{and they were chosen so as to incorporate the lexicon in different ways.}\amcomment{As mentioned, our approach is targeted settings where the target language does not have any related high-resource language to make use of. Since gathering data in different domains for truly low-resource languages is rather prohibitive, we instead use mBART: it is pre-trained on only 25 languages, thus enabling us to use some of left-out languages as \textit{low-resource}.} We evaluate all methods on a common test dataset. \amcomment{For evaluation, we use BLEU \cite{papineni-etal-2002-bleu} and ChrF \cite{popovic-2015-chrf}, as implemented by sacreBLEU \cite{post-2018-call}. We take ChrF as our main metric, as it focuses on the characters and would be more informative in case of translating into a low-resource language, that could be potentially morphologically rich.}
 
% We train mBART on the available resources -  parallel data (the Bible) and monolingual data (in the source language) - in different ways before finally testing it on a test dataset. All the following methods make use of a bilingual lexicon in some capacity. We then analyze the efficacy of different approaches for the task. 

% \noindent \textbf{Baselines}

$\bullet$ \textbf{mBART}: Our baseline is
%We use the 
the pre-trained and multilingual (25 languages) model  mBART, which 
%purportedly 
is said to generalize well to unseen languages \cite{liu-etal-2020-multilingual-denoising}. 


$\bullet$ \textbf{DALI}: We adapt the method from \citet{dali}, who extract a lexicon by mapping word embeddings from the source to the target language. They then use this lexicon to back-translate from the target monolingual data, by word-for-word replacement. The resulting texts are the pseudo-parallel data that are then used for training. 
%do not perform the lexicon induction as we 
We produce pseudo-parallel data using the same method, but assuming our lexicon is given. \amcomment{As we only have access to source-side monolingual data, we do forward-translation instead.}%\apedit{instead} assume the lexicon is given, \apedit{make word-for-word replacements,} and we do forward-translation. \apmargincomment{Please correct as necessary - what was missing here is a description of what part of this model we actually use.}
%as we only have access to source-side monolingual data. 


$\bullet$ \textbf{LeCA}: \citet{leca} append suggestions to the input to be used in the output. Their model uses a pointer-generator module to potentially copy from the input. Since the model updates just the probability of the next token by also considering copying from the input tokens, it is not a hard constraint. As we want to use our dictionary, we match their \textsc{Dictionary Constraint} setting, where suggestions are made by looking up source-side terms in a given dictionary. We implement this on top of the base mBART model as opposed to the basic Transformer. Note that LeCA was not originally proposed for low-resource scenarios, they do not use a pre-trained model, instead training the base Transformer model from scratch.


$\bullet$ \textbf{CPT}: \citet{liu-etal-2021-continual} continue pre-training mBART on mixed-language text, modifying the pre-training scheme of the model. They corrupt the text by replacing some terms with their translation in the new language, and the model is trained to reconstruct the original text. In our setting, we must use source-side monolingual text only, matching their \textsc{CPT w/ MLT (Src)} method. Note that in our experiments we translate from the high-resource language to the low-resource.%, and if it were the opposite and we were translating to the high-resource language, then using the target-side high-resource monolingual text for pre-training would correspond to their \textsc{CPT w/ MLT (Tgt)}, their main proposed method. 
%\apmargincomment{this last sentence can come out if we need space.}

$\bullet$ \textbf{Combined}: We experiment with merging the above methods: first, we  pre-train the model (CPT) and then train it with pseudo-parallel data (DALI) while using pointer-generators (LeCA). 




\input{tables/finalResults}

\section{Conclusion and Future Direction}

In this paper, we introduced a realistic setting that has been previously overlooked: domain adaptation for translation into a low-resource language from a high-resource language, with the available resources being in the form of a dictionary and monolingual texts in the high-resource language only. We tested some existing methods that could be applied to this task, all of which involve the dictionary. 
\st{Our results indicate that for the languages under study, these methods mostly fail to boost the performance to an acceptable level that would be considered useful.} \amcomment{Our results indicate that for the languages under study, the simplest approach studied here yields the best results. However, there is ample room for improvement; }
We \st{therefore} advocate for increased focus in this area of research within the NLP community, particularly for languages with data restricted to specific domains, as these languages are the most in need of domain adaptation and are often overlooked. 

==> sections/orig_Maltese.tex <==
%The example provided in 
\paragraph{Example } Table \ref{tab:example-mlt} 
%demonstrates some of these points. The 
shows a source sentence from the Maltese-medical test set and multiple outputs;
%of Maltese in the medical domain, 
this is the language-domain pair with the most significant performance boost. As expected, mBART and LeCA  translate in a religious tone. The same is true for CPT,
%as the Bible was the only parallel data it was trained on, 
but it also has copied certain words from the input - as it was a part of the reconstruction procedure in its pretraining.
It is important to emphasize that Maltese is a morphologically rich language, and the inflections are mostly discarded in the outputs of DALI and Combined; for example the words are more likely to be disjoint in their outputs than they are in the target (the first ``\textit{il o$\hbar$ra}'' vs ``\textit{l-o$\hbar$ra}'' in the target), or they can be in different forms (``\textit{huwa}'' vs ``\textit{hija}'').
Maltese at times has a different word order than that of English (
``\textit{il-mediċina  tal-g$\hbar$ajnejn}'' is translated as ``\textit{g$\hbar$ajn mediċina}'', which matches the order  of its English counterpart ``eye medicine''), and it is also more flexible. DALI and Combined produce word orders that closely follow the source language.
%, which could be a problem for many languages with different word orders.
